Minimax Model Learning

We present a novel off-policy loss function for learning a transition model in model-based reinforcement learning. Notably, our loss is derived from the off-policy policy evaluation objective with an emphasis on correcting distribution shift. Compared to previous model-based techniques, our approach allows for greater robustness under model misspecification or distribution shift induced by learning/evaluating policies that are distinct from the data-generating policy. We provide a theoretical analysis and show empirical improvements over existing model-based off-policy evaluation methods. We provide further analysis showing our loss can be used for off-policy optimization (OPO) and demonstrate its integration with more recent improvements in OPO.

==> sec-CI.tex <==
\section{OPE through Confidence Intervals (CI)}
\label{sec:CI}

We can inherit the confidence interval technique from \cite{jiang2020CI} to get an alternative minimax objective for model learning for OPE. In the proof of Lemma \ref{lem:DR}, we find that the MML loss has the following property for any $P \in \M$,
\begin{align*} 
J(\pi,P) - J(\pi,P^\ast) = \gamma L(w_{\pi}^{P},  V^{P^\ast}_{\pi}, P) 
% \quad \mbox{or} \\ 
%     J(\pi,P) - J(\pi,P^\ast)  = \gamma L(w_{\pi}^{P^\ast},  V^{P}_{\pi}, P)
\end{align*}
when the conditions of lemma \ref{lem:DR} hold. Rearranging, we get that 
\begin{equation*}
    J(\pi, P^\ast) = J(\pi,P) - \gamma L(w^{P}_\pi, V^{P^\ast}_\pi, P)
\end{equation*}
which implies
\begin{align*}
J(&\pi, P^\ast) = E_{D_{\pi_b} R P'}[\\
&w^{P}_\pi(s,a) (r - \gamma E_{x\sim P}[V^{P^\ast}_{\pi}(x)] - \gamma V^{P^\ast}_{\pi}(s')].
\end{align*}
Here we've used the fact that $J(\pi,P) = E_{(s,a,r) \sim \density{\pi}{P}(\cdot, \cdot) R(\cdot|s,a) }[r] = E_{D_{\pi_b} R}[w^{P}_\pi(s,a) r]$. This motivates a new loss
\begin{defn}[CI Loss] 
\begin{equation} 
    L_{\text{CI}}(w,V,P) \equiv E_{D_{\pi_b} R}[w r] - \gamma L(w,V,P)
\end{equation}
\end{defn}
From this we define the upper and lower bound of the confidence interval as
\begin{defn}[Upper and Lower CI]
\begin{equation*}
UB_P \equiv \inf_{P \in \M} \sup_{w \in \W,V \in \V} L_{CI}(w,V,P)   
\end{equation*}
\begin{equation*}
LB_P \equiv \sup_{P \in \M} \inf_{w \in \W,V \in \V} L_{CI}(w,V,P)
\end{equation*}
\end{defn}

% We may also write $LB_P = - \inf_{P \in \M} \sup_{w \in \W,V \in \V} (-L_{CI}(w,V,P))$. 
The upper and lower bound have the following properties:
\begin{thm}[Validity] \label{thm:validity} Let $P_{\inf} \in \M$ that which attains the infimum of $UB_{P}$ and $P_{\sup} \in \M$ that which attains the supremum of $LB_{P}$. Then
\begin{align*}
    UB_P &- J(\pi, P^\ast) \geq\\
    & \inf_P \sup_{w,V} \left( L_{CI}(w,V,P) - L_{CI}(w^{P_{\inf}}_\pi,V^{P^\ast}_\pi,P) \right)
\end{align*}
\begin{align*}
    J(\pi, &P^\ast) - LB_P \geq\\ &\inf_P \sup_{w,V} \left( L_{CI}(w^{P_{\sup}}_\pi,V^{P^\ast}_\pi,P) - L_{CI}(w,V,P)  \right)
\end{align*}
Furthermore, if $(w^{P}_\pi, V^{P^\ast}_\pi) \in \mathcal{W} \times \mathcal{V}$ for every $P \in \mathcal{M}$ then $LB_P \leq L(\pi, P^\ast) \leq UB_f$.
\end{thm}

The same result holds if we simultaneously swap $w^{P_{\inf}}_{\pi}$, $w^{P_{\sup}}_\pi$ for $w^{P^\ast}_{\pi}$ and $V^{P^\ast}_\pi$ for $V^{P_{\inf}}_{\pi}$, $V^{P_{\sup}}_\pi$. If we consider $w \cdot V$ as a single function of $(s,a,s')$ coming from $\W \times \V$, then $L(wV, P)$ is linear in $wV$. Hence we can write $L(w^{P_{\sup}}_\pi V^{P^\ast}_\pi - wV, P)$ and $L(wV - w^{P_{\inf}}_\pi V^{P^\ast}_\pi, P)$ where the terms $w^{P_{\sup}}_\pi V^{P^\ast}_\pi - wV$ and $wV - w^{P_{\inf}}_\pi V^{P^\ast}_\pi$ measure the degree of realizability of $wV$. Even if the confidence interval holds, it may only be useful if $UB_P \approx LB_P$, summarized as follows:

\begin{thm}[Tightness] 
\begin{equation*}
    UB_P - LB_P \leq 2 \inf_P \sup_{w,V} L(w,V,P)
\end{equation*}
If $P^\ast \in \M$ then $UB_P \leq LB_P$
\end{thm}

We have seen a few times that if $P^\ast \in \M$ then $L=0$, guaranteeing $UB_P \leq LB_P$. However, without the assumption of realizability of $\W,\V$ then $UB_P$ may be arbitrarily lower than $J(\pi,P^\ast)$ and $LB_P$ arbitrarily higher. Only when all three conditions are satisfied ($\W,\V$ realizable and $P^\ast \in \M$) do we have the interval collapse to a point $J(\pi,P^\ast) = UB_P = LB_P$.

Unfortunately, a closed from for the CI loss, like in Lemma \ref{lem:rkhs}, is not readily available \clv{is this true?}. Despite this, although stabilization may be necessary in practice, it is possible to compute the upper and lower bounds using an iterative approach similar to \cite{}. 

When a point estimate of $J(\pi, P^\ast)$ is desired, one may take the average of the upper and lower bounds. Surprisingly, this gives an estimate of the policy $\pi$ without ever having to run $\pi$ in any simulator $P \in \M$.

==> sec-OPE.tex <==
%!TEX root = ./icml.tex
\section{Off-Policy Policy Evaluation (OPE)}

% \begin{algorithm}[H]
% 	%\begin{small}
% 	\caption{Minimax Model Learning (MML) for off-policy policy evalution (OPE)} 
% 	\label{algo:mmlope}
% 	\begin{algorithmic}[1]
% 		\REQUIRE Pre-collected data set $D = \{ s_i,a_i,s^\prime\}_{i=1}^n \sim D_{\pi_b}(s,a)P^\prime(s^\prime|s_i,a_i)$. Function classes $\M, \W, \V$. 
% 		\REQUIRE $\pi$ is given
%         \STATE Initialize $P \in \M$.
% % 		\FOR{$k = 1,2,\ldots,K$}
% 		%\REPEAT
% 		\STATE $\widehat{P} \leftarrow \min_{P \in \M} \max_{w \in \W, V \in \V} L(w,V,P)^2$ \quad (Def \ref{loss:mml}) \\
% 		\quad\quad Using either (1) RKHS (Lemma \ref{lem:rkhs}) or \\
% 		\quad\quad \text{(2)} Alternating training between maximizing $w*V$ and minimizing $P$. \\
% 		\FOR{$k=1,2,\ldots,m$}
% 		\STATE Sample $s^k_0 \sim d_0$ \\
% 		\FOR{$t=0,1,\ldots,T-1$}
% 		\STATE $a^k_t \sim \pi(\cdot|s^k_t), r^k_t \sim \mathcal{R}(\cdot|s^k_t,a^k_t), s^k_{t+1} \sim \widehat{P}(\cdot|s^k_t,a^k_t)$ \\
% 		\ENDFOR
% 		\ENDFOR
% 		\ENSURE $J(\pi, \widehat{P}) = \frac{1}{m}\sum_{k=1}^m \sum_{t=0}^T \gamma^t r^k_t $
% 	\end{algorithmic}
% 	%\end{small}
% \end{algorithm}

In this section we examine how the MML error bounds 
OPE error.
%the OPE error given by algorithm \ref{algo:mmlope}. 
We assume there is some known $\pi$ for which we wish to know $J(\pi, P^\ast)$, despite only having data from $D_{\pi_b} P^\ast$. In other words, we are interested in the case when $\pi$ is different from $\pi_b$.


Suppose we take $J(\pi, \widehat{P})$ as the OPE estimate for $J(\pi, P^\ast)$. 
% As discussed in Section \ref{sec:mml}, with adequate control over $$\delta_{\pi}^{P,P^\ast} = |J(\pi, \widehat{P}) - J(\pi,P^\ast)|,$$ when realizability holds then $J(\pi, \widehat{P})$ is at most $\gamma \max_{w,V} \Loss(w,V,\widehat{P})$ away from the true value. 
Theorem \ref{lem:DR} quantifies the error we will incur by evaluating $\pi$ in $\widehat{P}$ instad of $P^\ast$, assuming the conditions hold. Therefore, $\widehat{P}$ is a reasonable proxy for $P$ for OPE. In this sense, MML is a principled method for model selection when the objective is OPE. For those interested in the sample complexity of the estimate see Appendix Thm \ref{thm:opeerror}.

% At this point we can make sense of what $\W$ and $\V$ function classes represent. Let $w_{\pi}^{P}(s,a) \equiv \frac{\density{\pi}{P}(s,a)}{D_{\pi_b}(s,a)}$ and $V^{P}_{\pi}$ as defined in the preliminaries. $w_{\pi}^{P}$ represents the shift from the state-action distribution $D_{\pi_b}$ to that of another distribution, in this case $\density{\pi}{P}(s,a)$. $V^{P}_{\pi}$ represents the value of running $\pi$ in $P$.

% The existence of $\frac{\density{\pi}{P}(s,a)}{D_{\pi_b}(s,a)}$ is only guaranteed when the data generating distribution is sufficiently exploratory, formalized as:
% \begin{assumption}[The dataset is exploratory]
% For every $P \in \M \cup \{P^\ast\} $, whenever $\density{\pi}{P}(s,a) >0 $ then $D_{\pi_b}(s,a) > 0$.
% \end{assumption}






% We wish to know that the in-simulator estimate is close to the true estimate $J(\pi, \widehat{P}) \approx J(\pi, P^\ast)$.
% It turns out that this is the case when $\W \times \V$ realizes either $(\frac{\density{\pi}{P}(s,a)}{D_{\pi_b}(s,a)}, \val{\pi}{P^{\ast}})$ or $(\frac{\density{\pi}{P^\ast}(s,a)}{D_{\pi_b}(s,a)}, \val{\pi}{P})$ for every $P \in \M$. Formally,

% \begin{lem}[Doubly-Robustness of Discriminators] \label{lem:DR}
% For a given policy $\pi$, if either $(w_{\pi}^{P}, V^{P^\ast}_{\pi}) \in \mathcal{W} \times \mathcal{V}$ or $(w_{\pi}^{P^\ast}, V^{P}_{\pi}) \in \mathcal{W} \times \mathcal{V}$ for all $P \in \M$ then
% \begin{equation}
%     |J(\pi,\widehat{P}) - J(\pi,P^\ast)| \leq \gamma \min_{P \in \M} \max_{w \in \W, V \in \V} |L(w,V,P)|
% \end{equation}
% \end{lem}

% \begin{rem} \label{rem:verifiability}
% In principle, $V^{P}_{\pi} \in \V$ can be verified for every $P \in \M.$ 
% \end{rem}

% If the exploratory state distribution $d_{\pi_b}$ and $\pi_b$ are known then $D_{\pi_b}$ is known. Since $\pi$ is also known, we can also verify that $w_{\pi}^{P} \in \W$ for every $P \in \M$.  Together with Remark \ref{rem:verifiability}, only one of $V^{P^\ast}_{\pi} \in \V$ or $w_{\pi}^{P^\ast} \in \W$ has to be realizable for Lemma \ref{lem:DR} to hold. For this reason, despite its traditional usage, we call this property doubly-robust. If these distributions are not known we may want to verify that at the very least $\frac{\density{\pi}{P}(s,a)}{E_n[D_{\pi_b}(s,a)]} \in \W$. \clv{why?}

% Additionally, despite the strong ``for all $P \in \M$'' condition in Lemma \ref{lem:DR}, we actually only need it to hold for the minimizer $\hat{P} = \arg\min_{P} \max_{w,V} |L(w,V,P)|$. Since we cannot know which $P \in \M$ will be the minimizer apriori, we will nevertheless have to verify that $w_{\pi}^{P} \in \W$ and $V^{P}_{\pi} \in \V$ for each $P \in \M$. 

% $J(\pi, \widehat{P})$ requires exact expectation of an infinite sum: $E_{d_0}[\sum_{t=0}^\infty \gamma^t r_t]$ where we collect $r_t$ by running $\pi$ in simulation $\widehat{P}$. Instead, we can only estimate an empirical average over a finite sum in $\widehat{P}_n$: $J_{T,m}(\pi, \widehat{P}_n) = \frac{1}{m} \sum_{j=1}^m \sum_{t=0}^T \gamma^t r^j_t$, where each $j$ indexes rollouts starting from $s_0 \sim d_0$ and the simulation is over $\widehat{P}_n$. Our OPE estimate is therefore bounded as follows:

% \begin{thm}\label{thm:opeerror}[OPE Error] Let the functions in $\V$ and $\W$ be uniformly bounded by $C_\V$ and $C_\W$ respectively. Assume the conditions of Lemma \ref{lem:DR} hold and $|\mathcal{R}| \leq \Rmax, \gamma \in [0,1)$. Then, with probability $1-\delta$, 
% \begin{align*}
% |&J_{T,m}(\pi,\widehat{P}_n) - J(\pi,P^\ast)| \leq \gamma \min_{P}\max_{w,V} |\Loss(w, V, P)| \\& + 4 \gamma \mathfrak{R}_n(\W, \V, \M) + \frac{2  \Rmax}{1-\gamma} \gamma^{T+1} \\
% & + \frac{2 \Rmax}{1-\gamma}\sqrt{\log(2/\delta)/(2m)} + 4 \gamma C_\W C_\V \sqrt{\log(2/\delta)/n}
% \end{align*}
% where $\mathfrak{R}_n(\W, \V, \M)$ is the Rademacher complexity of the function class 
% \begin{align*}
% \{(s,a,s') \mapsto   &w(s,a)(E_{x\sim P}[V(x)] - V(s')) : \\ &w \in \mathcal{W}, V \in \mathcal{V}, P \in \mathcal{\M}\}.
% \end{align*}
% \end{thm}

% \subsection{Comparison to Marginalized Importance Sampling}

% Significant attention has recently poured into marginalized importance sampling methods for OPE \cite{}. In essence these methods aim to replace importance sampling 
% $J(\pi, P^\ast) \approx \frac{1}{m} \sum_{k=1}^m \sum_{t=0}^T \prod_{i=0}^t \frac{\pi(a^k_i|s^k_i)}{\pi_b(a^k_i|s^k_i)} \gamma^t r^k_t$ with state(-action) density ratios 
% $J(\pi, P^\ast) \approx \frac{1}{Tm} \sum_{k=1}^m \sum_{t=0}^T \frac{\density{\pi}{P^\ast}(s^k_t, a^k_t) }{D_{\pi_b}(s^k_t, a^k_t)} r^k_t$. The term $ \frac{\density{\pi}{P^\ast}}{D_{\pi_b}}
% $ coincides with our term $w_{\pi}^{P^\ast}$. Specifically when $w_{\pi}^{P^\ast} \in \W$, Minimax Weight Learning (MWL, \cite{Uehara202minimax}) should return a perfect estimate of $J(\pi, P^\ast)$, assuming exact expectations. Our method (with properly specified $\V$) is guaranteed to return an approximately correct value, even with exact expectations, but comes with the added flexibility of a model. In the case when $w_{\pi}^{P^\ast} \not\in \W$ but $(w_{\pi}^{\widehat{P}}, V_{\pi}^{P^\ast}) \in \W \times \V$, both MML and MWL will return approximately correct values. However, in such a situation MQL (another minimax OPE method from \cite{Uehara2020minimax}) should give zero error.



==> sec-alternative.tex <==
\section{MML and Residual Dynamics}

Suppose we already had some baseline model $P_0$ of $P^\ast$. Alternatively, we may view this as the real world starting with (approximately) known dynamics $P_0$ and drifting to $P^\ast$. We can modify MML to incorporate knowledge of $P_0$ to find the residual dynamics that are distributionally and decision-aware as follows:
\begin{defn}\label{loss:mml}[Residual MML Loss] For $w \in \W, V \in \V, P \in \M$,
\begin{align*} 
    &\Loss(w,V,P) = E_{(s,a,s') \sim D_{\pi_b}(\cdot,\cdot) P^\ast(\cdot|s,a)} [w(s,a) \;\cdot
    \\&\left( E_{x\sim P_0(\cdot|s,a)}[\frac{P_0(x|s,a)-P(x|s,a)}{P_0(x|s,a)} V(x)] - V(s') \right)]
\end{align*}
\end{defn}

==> sec-computation.tex <==
\section{Computational Considerations}

A discussion about computational issues can be found in Appendix \ref{app:compconsiderations}. We show there that, like \cite{uehara2019minimax}, we can simplify the minimax problem to minimization in a closed form when $\W\V$ correspond to a reproducing kernel Hilbert space (RKHS). We also show that the entire minimax procedure has a closed form when the classes consist of only linear functions (e.g. tabular setting).




==> sec-experiments2.tex <==
 \makeatletter
\newcommand{\customlabel}[3]{%
%%% without hyperref: only 2 arguments instead of 5
   \protected@write \@auxout {}{\string \newlabel {#1}{{\ref{#2}~(#3)}{\thepage}{}{}{}} }%
%   \protected@write \@auxout {}{\string \newlabel {sub@#1}{{#3}{\thepage}{Subfigure #2 (#3)\relax}{}{}} }%
}
\makeatother


\begin{figure*}[]
    \centering     %%% not \center
% \hfill
%     \customlabel{fig:car_screenshot}{fig:car}{first}%
%         \includegraphics[width=1.2in]{figs/lqr_single_ope_edited.pdf}
\hfill%
    \customlabel{fig:LQR_MML_vs_rest}{fig:lqr}{left}%
        \includegraphics[width=.45\linewidth]{figs/lqr_single_ope_edited.pdf}
\hfill% 
    \customlabel{fig:LQR_verifiability}{fig:lqr}{right}%
        \includegraphics[width=.45\linewidth]{figs/V_validation_edited.pdf}
% \hfill% 
%     \customlabel{fig:car_fqe}{fig:car}{fourth}%
%         \includegraphics[width=1.7in]{lqr_single_ope_edited.pdf}
        \vspace{-0.1in}
\caption{\emph{LQR}.
             \emph{(Left, OPE Error)} MML finds the $P \in \M$ with the lowest OPE error as $\M$ gets richer. Since calculations are done in expectation, no error bars are included. 
             \emph{(Right, Verifiability)} The OPE error (smoothed) increases with misspecification in $\V$ parametrized by $\epsilon$, the expected MSE between the true $V^{P^\ast}_{\pi} \not\in \V$ and the approximated $\widehat{V}^{P^\ast}_{\pi} \in \V$. Nevertheless, directionally they all follow the same trajectory as $\M$ gets richer.
             }
\label{fig:lqr}
\end{figure*}


\section{Experiments}
\label{sec:experiments}


In our experiments, we seek to answer the following questions: (1) Does MML prefer models that minimize the OPE objective? (2) What can we expect when we have misspecification in $\V$? (3) How does MML perform against MLE and VAML in OPE? (4) Does our approach complement modern offline RL approaches?  For this last question, we consider integrating MML with the recently proposed MOREL \citep[]{kidambi2020morel} approach for offline RL. See Appendix \ref{app:morel} for details on MOREL.





% \begin{figure*}[ht] 
% %   \label{ fig7} 
%   \begin{minipage}[b]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/lqr_single_ope_edited.pdf} 
%     \caption{\textit{(OPE Error in LQR) As the class $\M$ gets richer, MML takes advantage and finds the simulator $P \in \M$ with the lowest OPE error. Since calculations are done in expectation, no error bars are included. 
%     % \yisong{LQR?}
%     } }
%      \label{fig:OPE}
%     \vspace{4ex}
%   \end{minipage}%%
%   \begin{minipage}[b]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/V_validation_edited.pdf} 
%     % \caption{\textit{(OPE Error in LQR) As the class $\M$ gets richer, MML takes advantage and finds the simulator $P \in \M$ with the lowest OPE error. Since calculations are done in expectation, no error bars are included. }}
%     \vspace{4ex}
%   \caption{\textit{(OPE Error in LQR) As the class $\M$ gets richer, MML takes advantage and finds the simulator $P \in \M$ with the lowest OPE error. Since calculations are done in expectation, no error bars are included. 
%     % \yisong{LQR?}
%     } }
%   \end{minipage} 
%   \begin{minipage}[b]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/lqr_single_ope_edited.pdf} 
%     \caption{DFT, Initial condition} 
%     \vspace{4ex}
%   \end{minipage}%% 
%   \begin{minipage}[b]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/lqr_single_ope_edited.pdf} 
%     \caption{DFT, rupture} 
%     \vspace{4ex}
%   \end{minipage} 
% \end{figure*}


% \begin{figure*}[!ht]
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/lqr_opo.pdf}
% \endminipage\hfill
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/lqr_ope.pdf}
% %   \caption{Toy-Graph MDP with stochastic transitions amd rewards comparison. $\pi(a=0)=.2, \pi_e(a=0)=.8$. $N=1024$. See Table \ref{tab:TG_MDP_T4_N1024_stochT_stochR_pi0_20_pi1_80} and Table \ref{tab:TG_MDP_T16_N1024_stochT_stochR_pi0_20_pi1_80}}
% %   \label{fig:ToyGraphStochMDP}
% \endminipage\hfill
% \vspace{-0.1in}
% \caption{Left: \textit{(LQR OPO)
% VAML and MLE immediately take on the $P$ such that $\pi^\ast_{P^\ast} = \pi^\ast_{P}$, leaving zero OPO error. As MML has to be robust to larger $|\W|, |\V|$, it does eventually coincide with the rest, which verifies that MML and MLE coincide in LQR OPO.}
% \textit{(LQR OPE) VAML and MLE take on significantly larger OPE error compared to MML both in the worst-case scenario (max) and on average (mean) while the sets $|\W|$ and $|\V|$ remain small. Eventually all the methods coincide, as expected.
% }}
%  \label{fig:lqr}
%  \vspace{-.15in}
% \end{figure*}https://www.overleaf.com/project/5e754e88bb95ea0001a3df23

% \begin{figure}[!ht]
% % \minipage{.5\textwidth}
% %   \includegraphics[width=\linewidth]{../figs/tabular_P_default.png}
% % \endminipage\hfill
% % \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{figs/lqr_single_ope_edited.pdf}
% % \endminipage\hfill
% \vspace{-0.3in}
% \caption{\textit{(OPE Error in LQR) As the class $\M$ gets richer, MML takes advantage and finds the simulator $P \in \M$ with the lowest OPE error. Since calculations are done in expectation, no error bars are included. 
% % \yisong{LQR?}
% } }
%  \label{fig:OPE}
%  \vspace{-.1in}
% \end{figure}


% \textbf{Environment and Setup.} The LQR domain is a 1D stochastic environment with true dynamics: $P^\ast(s'|s,a) = s - .5 a + w^\ast$ where $w^\ast \sim N(0,.01)$. The reward function is $R(s,a) = -(s+a)$ and $\gamma = .9$. 
% We use a finite class $\M$ consisting of all deterministic policies $\M = \{P_x(s'|s,a) = (1 + x/10) s - (.5 + x/10) a | x \in [0, M]\}$ where we vary $M \in \{2,3,\ldots, 19\}.$ We wish to evaluate $\pi(a|s) = N(1.3 s, .01)$. We calculate $\W$ and $\V$ using our calculations from Section \ref{subsec:lqr} and make sure $V^P_{\pi} \in \V$ for all $P \in \M$, and $W^{P^\ast}_{\pi} \in \W$. With the simplicity of this environment, we are able to run all our calculations exactly (in expectation). 

% \begin{rem}\label{rem:lqr} While $P^\ast \not\in \M$, we do have $\pi^\ast_{P^\ast} \in \Pi$ since $\pi^\ast_{P^\ast} = \pi^\ast_{P_0}$ where $P_0(s'|s,a) = s - .5 a.$ This follows from the fact that, in LQR, models with identical transition dynamics (up to noise) have identical optimal policies.
% \end{rem}

\subsection{Brief Environment Description and Experimental Setup}

We perform our experiments in three different domains. A thorough description of the environments, setup and hyperparameters is given in Appendix \ref{app:experiments}.

\textbf{Linear-Quadratic Regulator (LQR).} 
% The LQR domain is a 1D environment with stochastic dynamics $P^\ast(s'|s,a)$. We use a finite class $\M$ consisting of deterministic policies.
The LQR domain is a 1D stochastic environment with stochastic dynamics: $P^\ast(s'|s,a) = s - .5 a + w^\ast$ where $w^\ast \sim N(0,.01^2)$. We let $x_0 \sim N(1, .1^2)$. The reward function is $R(s,a) = -(s+a)$ and $\gamma = .9$.

We use a finite class $\M$ consisting of all deterministic models $\M = \{P_x(s'|s,a) \equiv (1 + x/10) s - (.5 + x/10) a | x \in \{0,\ldots,M\}\}$ where we vary $M \in \{2,3,\ldots, 19\}$ in the experiment.   We write $(A^\ast, B^\ast) = P_0(s'|s,a) = A^\ast s + B^\ast a$, the deterministic version of $P^\ast$. 

We ensure $V^P_{\pi} \in \V$ for all $P \in \M$ by solving the equations in Appendix Lemma \ref{lem:VQuad_LQR}. We ensure $W^{P^\ast}_{\pi} \in \W$ using Appendix Equation \eqref{eq:lqr_dpi}. 

\textbf{Cartpole \citep[]{OpenAIgym}.} 
% The reward function is modified to be a function of angle and location rather than 0/1 to make the OPE problem more challenging. Each $P \in \M$ is a parametrized NN that outputs a mean, and logvariance representing a normal distribution around the next state.
We use the standard Cartpole benchmark (OpenAI, \cite{OpenAIgym}). The state space is a tuple $(x,\dot{x}, \theta, \dot{\theta})$ representing the position of the cart, velocity of the cart, angle of the pole and angular velocity of the pole, respectively. The action space is discrete given by pushing the car to the left or right. We add $N(0,.001^2)$ Gaussian noise to each component of the state to make the dynamics stochastic.  We consider the infinite horizon setting with $\gamma=.98$. The reward function is modified to be a function of angle and location  $R(s,\theta) = (2 - \theta / \theta_{\max}) * (2 - s / s_{\max}) - 1$) rather than 0/1 to make the OPE problem more challenging. 

Each $P(s'|s,a) \sim \mathcal{N}(\mu(s,a), \sigma(s,a)) \in \M$, where a NN outputs a mean, and logvariance representing a normal distribution around the next state. Each model has two hidden layers with $64$ units each and ReLU activation followed by a final linear layer. 

We model the class $\W\V$ as a RKHS as in Lemma \ref{lem:rkhs} with an RBF kernel. We do the same for VAML. The RKHS kernel we use for MML is given by $K(s,a,s') = K_1(s) K_2(a) K_3(s')$ where $K_i$ are Gaussian Radial Basis Function (RBF) kernels with a bandwidth equal to the median of the pair-wise distances for each coordinate ($s,a,s'$ independently) over the batch.

\textbf{Inverted Pendulum (IP) \citep[]{laypy}.}  
This IP environment has a Runge-Kutta(4) integrator rather than Forward Euler (Runge-Kutta(1)) as in OpenAI \citep[]{OpenAIgym}, producing significantly more realistic data. 
% Each $P \in \M$ is a deterministic model parametrized with a neural network.
The state space is a tuple $(\theta, \dot{\theta})$ representing the  angle of the pole and angular velocity of the pole, respectively. The action space $\mathcal{A} = \R$ is continuous representing a clockwise or counterclockwise force. The reward function is a clipped quadratic function $R([\theta, \dot{\theta}], a) = \min(((\theta + \pi) \mod 2\pi - \pi)^2 + .1 \dot{\theta}^2 + .001 u^2, 100)$. 
We consider the infinite horizon setting with $\gamma=.98$. 
% This IP environment has a Runge-Kutta(4) integrator \citep[]{laypy} rather than Forwrd Euler and, thus, produces more realistic data.
The mass of the rod is $.25$ and the length $.5$.

We use $P(s'|s,a) = \frac{1}{4}\sum_{i=1}^4 P_i(s'|s,a)$ where each $P_i$ is a feed-forward  deterministic model given by a NN with two layers of $16$ units with Tanh activation followed by a final linear layer. 

The $\W\V$ class is an RKHS kernel given by $K(s,a,s') = K_1(s) K_2(a) K_3(s')$ where $K_i$ are Gaussian Radial Basis Function (RBF) kernels with a bandwidth equal to $1$. 

\subsection{Results}

\textbf{\textit{Does MML prefer OPE?}}  We vary the size of the model class Figure \ref{fig:LQR_MML_vs_rest} testing to see if MML will pick up on the models which have better OPE performance. When the sizes of $|\M|$ are small, each method selects $(A^\ast, B^\ast)$ (e.g. $P(s'|s,a) = A^\ast s + B^\ast a$), the deterministic version of the optimal model. However, as we increase the richness of $\M$, MML begins to pick up on models that are able to better evaluate $\pi$.

Two remarks are in order. In LQR, policy optimization in $(A^\ast, B^\ast)$ coincides with policy optimization in $P^\ast$. Therefore, if we tried to do policy optimization in our selected model then our policy would be suboptimal in $P^\ast$. Secondly, MML deliberately selects a model other than $(A^\ast, B^\ast)$ because a good OPE estimate relies on appoximating the contribution from the stochastic part of $P^\ast$.


% trying to fit the noise $w^\ast$ in $P^\ast$ precisely because $P \in \M$ are all deterministic. %In other words, MML selects a model deliberately different than $P_0$ because nearly half the time predicts larger states than  would return. 

\textbf{\textit{A Tradeoff?}}
There is a trade-off between the OPE objective and the OPO objective. MML's preference is dependent on the capacities of $\M, \W, \V$. Figure \ref{fig:LQR_MML_vs_rest} illustrates OPE is preferred for $\W$ fixed. Appendix Figure \ref{fig:LQR_MML_vs_rest_OPO} explores the OPO objective and shows that if we increase $\W$ then OPO becomes favored. One interpretation of this is we are asking MML to be robust to many more OPE problems as $|\W|\uparrow$ and therefore the performance on any single one decreases but overall we are more likely to be able to do OPO. 

\textbf{\textit{Misspecification and Verifiability?}} To check verifiability in practice, we would run $\pi$ in a few $P \in \M$ and calculate $V^{P}_\pi$. Then we would check if $V^{P}_\pi \in \V$ by fitting $\widehat{V}^P_{\pi}$ and measuring the empirical gap $E[(\widehat{V}_\pi^{P} - V_\pi^{P})^2] = \epsilon^2$. \textit{Do we have to close this gap?}

Figure \ref{fig:LQR_verifiability} shows how MML performs when $V_\pi^{P} \not\in \V$ but we do have $\widehat{V}_\pi^{P}(s) = V_\pi^{P}(s) + \mathcal{N}(0,\epsilon) \in \V$. Since $E[(\widehat{V}_\pi^{P} - V_\pi^{P})^2] = \epsilon^2$ then $\epsilon$ is the root-mean squared error between the two functions. Directionally all of the errors go down as $|\M|\uparrow,$ however it is clear that $\epsilon$ has a noticeable effect. We speculate that if this error not distributed around zero and instead is dependent on the state then the effects can be worse. 

\textbf{\textit{MML for OPE?}} In addition to Figure \ref{fig:LQR_MML_vs_rest},  Figure \ref{fig:OPE} also illustrates that our method outperforms the other model-learning approaches in OPE. The environment and reward function is challenging, requiring function approximation. This further validates that MML is a good choice for model-learning with an OPE objective. Despite the added complexity of solving a minimax problem, doing so gives nearly an order of magnitude improvement over MLE and many orders over VAML. 

% The performance boost is due to the improvement in distributional robustness and decision-awareness over VAML and MLE respectively.  
%over previous value-aware work (VAML) is not distributionally robust and that MLE suffers from lacking decision-awareness. 

% \begin{figure*}[]
%     \centering     %%% not \center
% % \hfill
% %     \customlabel{fig:car_screenshot}{fig:car}{first}%
% %         \includegraphics[width=1.2in]{figs/lqr_single_ope_edited.pdf}
% \hfill%
%     \customlabel{fig:OPE}{fig:OPE}{left}%
%         \includegraphics[width=.45\linewidth]{figs/ope_cartpole_edited.pdf}
% \hfill% 
%     \customlabel{fig:OPE2}{fig:OPE2}{right}%
%         \includegraphics[width=.45\linewidth]{figs/ope_cartpole_edited.pdf}
% % \hfill% 
% %     \customlabel{fig:car_fqe}{fig:car}{fourth}%
% %         \includegraphics[width=1.7in]{lqr_single_ope_edited.pdf}
%         \vspace{-0.1in}
% \caption{\emph{LQR}.
%              \emph{(Left, OPE Error)} MML finds the $P \in \M$ with the lowest OPE error as $\M$ gets richer. Since calculations are done in expectation, no error bars are included. 
%              \emph{(Right, Verifiability)} The OPE error (smoothed) increases with misspecification in $\V$ parametrized by $\epsilon$, the expected MSE between the true $V^{P^\ast}_{\pi} \not\in \V$ and the approximated $\widehat{V}^{P^\ast}_{\pi} \in \V$. Nevertheless, directionally they all follow the same trajectory as $\M$ gets richer.
%              }
% \label{fig:lqr2}
% \end{figure*}






\begin{figure}[!t]
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/tabular_P_default.png}
% \endminipage\hfill
% \minipage{.5\textwidth}
  \includegraphics[width=\linewidth]{figs/ope_cartpole_edited.pdf}
% \endminipage\hfill
\vspace{-0.3in}
\caption{\textit{ (Cartpole, OPE Error) Comparison of model-based approaches for OPE with function-approx.} \textit{Lower is better. MML outperforms others. 
Not pictured: traditional model-free methods such as IS/PDIS have error of order 3-8.
% validating that VAML is not distributionally robust and that MLE is not decision-aware. 
}}
 \label{fig:OPE}
 \vspace{-.1in}
\end{figure}

% \subsection{Inverted Pendulum}
% \textbf{Environment and Setup.} We use a Inverted Pendulum (IP) benchmark (\citep[]{???}). The \citep[]{???} IP we used has a Runge-Kutta(4) integrator rather than Forward Euler (Runge-Kutta(1)), which makes it produce significantly more realistic data.

% We consider the infinite horizon setting with $\gamma=.98$. The reward function is a clipped quadratic function $R([\theta, \dot{\theta}], a) = \min(((\theta + \pi) \mod 2\pi - \pi)^2 + .1 \dot{\theta}^2 + .001 u^2, 100)$. Each $P \in \M$ is a deterministic model parametrized with a neural network. We generate the behavior data using a noisy feedback-linearized controller: $\pi_b(a|s)$ is uniformly random with probability $.3$ and is a feedback-linearized LQR controller with probability $.7$. We truncate all rollouts at $200$ time steps. We model the class $\W\V$ as a RKHS as in Lemma \ref{lem:rkhs} with an RBF kernel. We do the same for VAML. Further details can be found in  Appendix \ref{app:experiments}.

% Significant research effort has gone into state-of-the-art methods for offline policy optimization, dealing mostly with uncertainitly quantification \citep[]{kidambi2020morel, DeisenrothPILCO2011, Chua2018PETS, Jenner2019MBPO}. 


% \textbf{OPO Setup.} We input each of MML, VAML and MLE into into MOREL \citep[]{kidambi2020morel} to test how these loss functions perform. Our contribution is orthogonal from that of MOREL; MOREL penalizes the policies for venturing too far away from $D$ after the model has already been learned. \clv{$\leftarrow$want to say our result is orthogonal to MOREL.... clean up}

%  \begin{algorithm}[H]
% 	%\begin{small}
% 	%\renewcommand{\thealgorithm}{}
% 	\caption{OPO Algorithm (based on MOREL \citep[]{kidambi2020morel}) } 
% 	\label{algo:main_morel}
% 	\begin{algorithmic}[1]
%     	\REQUIRE $D = D_{\pi_b}P^\ast$
% 	    \STATE Learn an ensemble of dynamics $P_1,\ldots,P_4 \in \M$ using MML, VAML, MLE
% 	    \STATE Construct an $\alpha$-USAD, $U^\alpha: \State \times \A \to \{\text{TRUE},\text{FALSE}\}$ where $
% 	    \alpha = Median(\{ \|P_j(s,a) - s'\|_2 : j \in [1,\ldots,4], (s,a,s') \subset D\}).$ See Appendix \ref{app:morel} for the definitions.
% 	    \STATE Construct a pessimistic MDP $\mathcal{M}$ (see Appendix \ref{app:morel}) with $P(s,a) = \frac{1}{4} \sum_{i=1}^{4} P_i(s,a)$.
% 	    \STATE $\widehat{\pi} \leftarrow \text{PPO}(\mathcal{M})$ (Best of 3) \citep[]{Schulman17PPO}
% 	\end{algorithmic}
% 	%\end{small}
% \end{algorithm}

 \begin{algorithm}[H]
	%\begin{small}
	%\renewcommand{\thealgorithm}{}
	\caption{OPO Algorithm (based on MOREL \citep[]{kidambi2020morel}) } 
	\label{algo:main_morel}
	\begin{algorithmic}[1]
    	\REQUIRE $D$, $\Loss$ among \{MML, MLE, VAML\}
    % 	\vspace{-.4cm}
	    \STATE Learn an ensemble of dynamics $P_1,\ldots,P_4 \in \M$ using $P_i = \arg\min_{P \in \M} \Loss(D)$
	   % \STATE Construct an $\alpha$-USAD where $
	   % \alpha = Median(\{ \|P_j(s,a) - s'\|_2 : j \in [1,\ldots,4], (s,a,s') \subset D\}).$ See Appendix \ref{app:morel} for the definitions.
	    \STATE Construct a pessimistic MDP $\mathcal{M}$ (see Appendix \ref{app:morel}) with $P(s,a) = \frac{1}{4} \sum_{i=1}^{4} P_i(s,a)$.
	    \STATE $\widehat{\pi} \leftarrow \text{PPO}(\mathcal{M})$ (Best of 3) \citep[]{Schulman17PPO}
	\end{algorithmic}
	%\end{small}
\end{algorithm}


\textbf{\textit{MML for OPO?}} We integrate MML, VAML, and MLE with MOREL as in Algorithm \ref{algo:main_morel}. Consequently, Figure \ref{fig:OPO} shows that MML performs competitively with the other methods, achieving near-optimal performance as the number of trajectories increases. MML has good performance even in the low-data regime, whereas other methods perform worse than $\pi_b$. Performance in the low-data regime is of particular interest since sample efficiency is highly desirable.

Algorithm \ref{algo:main_morel} forms a pessimistic MDP where a policy is penalized if it enters a state where there is disagreement between $P_1,\ldots,P_4$. Given that MML performs well in low-data, we can reason that MML produces models with support that stays within the dataset $D$ or generalize well slightly outside this set. The other models poor performance is suggestive of incorrect over-confidence outside of $D$ and PPO produces a policy which takes advantage of this.


\begin{figure}[!ht]
\vspace{-0.27in}
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/tabular_P_default.png}
% \endminipage\hfill
% \minipage{.5\textwidth}
  \includegraphics[width=\linewidth]{figs/opo_IP_edited.pdf}
% \endminipage\hfill
\vspace{-0.3in}
\caption{\textit{ (Invert. Pend., OPO Performance) Comparison of model-based approaches for OPO with function-approx using Algorithm \ref{algo:main_morel}. Higher is better.} \textit{MML performs competitively even in low data regimes.
}}
 \label{fig:OPO}
 \vspace{-.1in}
\end{figure}

% \subsection{Learning}

% \subsubsection{Environment Description}
% We examine learning a good policy in Cartpole with a horizon of $200$ and a standard $0/1$ reward function. We collect data by running a near-perfect trained model (via TRPO) modified to take random actions with probability $1-\alpha$.  

% \subsubsection{Result}
% Figure \ref{fig:learning}(Left) illustrates the quality of policies learned over the learning iterations. What we notice is in general these methods are all fairly competitive with eachother in this environment. Different methods may converge faster than others but what we notice is that this is a function of how quickly the (log)variance converges. As we see in Figure \ref{fig:learning}(Right), after only 2 iterations the mean of MML seems to accurately predict the next state, but it takes a bit more iterations for the variance to decrease sufficiently. \clv{more} 


% \begin{figure*}[!ht]
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/learning_curve.png}
% \endminipage\hfill
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/current_to_next_state.png}
% \endminipage\hfill
% \vspace{-0.1in}
% \caption{\textit{ Learning a good policy in Cartpole.} Left: \textit{The methods converge at different rates, all fall into relatively the same neighborhood.} Right: \textit{After just 2 iterations, MML already makes accurate mean predictions, but the variance is too large to learn. After many more iterations, thhe variance decreases enough that a good policy can be learned.
% }}
%  \label{fig:learning}
%  \vspace{-.1in}
% \end{figure*}

==> sec-experiments_old.tex <==
\section{Experiments}
\label{sec:experiments}

In our experiments, we seek to answer the following questions: (1) Does MML prefer models that minimize the OPE objective? (2) What can we expect when we have misspecification in $\V$ (3) How does MML perform against MLE and VAML in both OPE and OPO? Is MML a reasonable method for OPE/OPO model selection?  We perform our experiments in three different domains: an LQR environment, OpenAI Mountain Car \citep[]{OpenAIgym}, and an Inverted Pendulum environment \citep[]{???}. 

\subsection{LQR}

% \begin{figure*}[!ht]
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/lqr_opo.pdf}
% \endminipage\hfill
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/lqr_ope.pdf}
% %   \caption{Toy-Graph MDP with stochastic transitions amd rewards comparison. $\pi(a=0)=.2, \pi_e(a=0)=.8$. $N=1024$. See Table \ref{tab:TG_MDP_T4_N1024_stochT_stochR_pi0_20_pi1_80} and Table \ref{tab:TG_MDP_T16_N1024_stochT_stochR_pi0_20_pi1_80}}
% %   \label{fig:ToyGraphStochMDP}
% \endminipage\hfill
% \vspace{-0.1in}
% \caption{Left: \textit{(LQR OPO)
% VAML and MLE immediately take on the $P$ such that $\pi^\ast_{P^\ast} = \pi^\ast_{P}$, leaving zero OPO error. As MML has to be robust to larger $|\W|, |\V|$, it does eventually coincide with the rest, which verifies that MML and MLE coincide in LQR OPO.}
% \textit{(LQR OPE) VAML and MLE take on significantly larger OPE error compared to MML both in the worst-case scenario (max) and on average (mean) while the sets $|\W|$ and $|\V|$ remain small. Eventually all the methods coincide, as expected.
% }}
%  \label{fig:lqr}
%  \vspace{-.15in}
% \end{figure*}https://www.overleaf.com/project/5e754e88bb95ea0001a3df23

\begin{figure}[!ht]
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/tabular_P_default.png}
% \endminipage\hfill
% \minipage{.5\textwidth}
  \includegraphics[width=\linewidth]{figs/lqr_single_ope_edited.pdf}
% \endminipage\hfill
\vspace{-0.3in}
\caption{\textit{(OPE Error in LQR) As the class $\M$ gets richer, MML takes advantage and finds the simulator $P \in \M$ with the lowest OPE error. Since calculations are done in expectation, no error bars are included. 
% \yisong{LQR?}
} }
 \label{fig:OPE}
 \vspace{-.1in}
\end{figure}


\textbf{Environment and Setup.} The LQR domain is a 1D stochastic environment with true dynamics: $P^\ast(s'|s,a) = s - .5 a + w^\ast$ where $w^\ast \sim N(0,.01)$. The reward function is $R(s,a) = -(s+a)$ and $\gamma = .9$. 
We use a finite class $\M$ consisting of all deterministic policies $\M = \{P_x(s'|s,a) = (1 + x/10) s - (.5 + x/10) a | x \in [0, M]\}$ where we vary $M \in \{2,3,\ldots, 19\}.$ We wish to evaluate $\pi(a|s) = N(1.3 s, .01)$. We calculate $\W$ and $\V$ using our calculations from Section \ref{subsec:lqr} and make sure $V^P_{\pi} \in \V$ for all $P \in \M$, and $W^{P^\ast}_{\pi} \in \W$. With the simplicity of this environment, we are able to run all our calculations exactly (in expectation). 

\begin{rem}\label{rem:lqr} While $P^\ast \not\in \M$, we do have $\pi^\ast_{P^\ast} \in \Pi$ since $\pi^\ast_{P^\ast} = \pi^\ast_{P_0}$ where $P_0(s'|s,a) = s - .5 a.$ This follows from the fact that, in LQR, models with identical transition dynamics (up to noise) have identical optimal policies.
\end{rem}

\textbf{Results.} \yisong{Figure 2?}  When the sizes of $|\M|$ are small, each method selects $P_0(s'|s,a)$. However, as we increase the richness of $\M$, MML begins to pick up on models that are able to better evaluate $\pi$. At some point it levels off. The reason for levelling off is that our grid over $\M$ is too coarse and picking a different model would either have higher OPE error (or unbounded error). 

Two remarks are in order. First, the model MML selects is not $P_0$. If we tried to do policy optimization in our selected model then our policy would be suboptimal in $P^\ast$. Secondly, the model MML selects is trying to fit the noise $w^\ast$ in $P^\ast$ since $P \in \M$ are all deterministic. In other words, MML selects a model deliberately different than $P_0$ because nearly half the time $w^\ast$ causes larger states than $P_0$ would return.

% give larger errors but are still stable to get good OPE error.  
In Appendix \ref{sec:experiments} we explore the OPO objective instead. There we can also see that MML is able to pick the best OPO model after $\M$ becomes rich enough while MML is required to be robust to increased $\W,\V$. 






\subsection{Cartpole}
\textbf{Environment and Setup.} We use the standard Cartpole benchmark (OpenAI, \cite{OpenAIgym}). We consider the infinite horizon setting with $\gamma=.98$. The reward function is modified to be a function of angle and location ($(2 - \theta / \theta_{\max}) * (2 - s / s_{\max}) - 1$) rather than 0/1 to make the OPE problem more challenging. Each $P \in \M$ takes the form $s' \sim \mathcal{N}(\mu(s,a), \sigma(s,a))$, where a NN outputs a mean, and logvariance representing a normal distribution around the next state. We generate the behavior and target policy using a near-perfect DDQN-based policy $Q$ with a final softmax layer and adjustable parameter $\tau$: $\pi(a|s) \propto \exp(Q(s,a)/\tau).$ The behavior policy has $\tau = 1$, while the target policy has $\tau = 1.5$. We truncate all rollouts at $1000$ time steps and we calculate the true expected value using the MC average of $10000$ rollouts. We model the class $\W\V$ as a RKHS as in Lemma \ref{lem:rkhs} with an RBF kernel. We do the same for VAML. Further details can be found in  Appendix \ref{app:experiments}.

We compare the methods using the log-relative MSE metric: $\log(\frac{(J(\pi,\widehat{P}) - J(\pi,P^\ast))^2}{(J(\pi_b,P^\ast) - J(\pi,P^\ast))^2})$, which is negative when the OPE estimate $J(\pi, \widehat{P})$ is superior to the on-policy estimate $J(\pi_b, \widehat{P})$. The more negative, the better the estimate. We take the average over $5$ trials and plot the log-relative MSE with standard error.

\textbf{Results.} As seen in Figure \ref{fig:OPE}, our method outperforms the other model-learning approaches in OPE. This environment and reward function is challenging, requiring function approximation. This further validates that MML is a good choice for model-learning with an OPE objective. Despite the added complexity of solving a minimax problem, doing so gives nearly an order of magnitude improvement over MLE and many orders over VAML. 

% The performance boost is due to the improvement in distributional robustness and decision-awareness over VAML and MLE respectively.  
%over previous value-aware work (VAML) is not distributionally robust and that MLE suffers from lacking decision-awareness. 

\begin{figure}[!ht]
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/tabular_P_default.png}
% \endminipage\hfill
% \minipage{.5\textwidth}
  \includegraphics[width=\linewidth]{figs/ope_cartpole.pdf}
% \endminipage\hfill
\vspace{-0.3in}
\caption{\textit{ Comparison of model-based approaches for OPE with function-approx (Cartpole).} \textit{MML outperforms other model-based methods. 
% validating that VAML is not distributionally robust and that MLE is not decision-aware. 
}}
 \label{fig:OPE}
 \vspace{-.1in}
\end{figure}

\subsection{Inverted Pendulum}
\textbf{Environment and Setup.} We use a Inverted Pendulum (IP) benchmark (\citep[]{???}). The \citep[]{???} IP we used has a Runge-Kutta(4) integrator rather than Forward Euler (Runge-Kutta(1)), which makes it produce significantly more realistic data.

We consider the infinite horizon setting with $\gamma=.98$. The reward function is a clipped quadratic function $R([\theta, \dot{\theta}], a) = \min(((\theta + \pi) \mod 2\pi - \pi)^2 + .1 \dot{\theta}^2 + .001 u^2, 100)$. Each $P \in \M$ is a deterministic model parametrized with a neural network. We generate the behavior data using a noisy feedback-linearized controller: $\pi_b(a|s)$ is uniformly random with probability $.3$ and is a feedback-linearized LQR controller with probability $.7$. We truncate all rollouts at $200$ time steps. We model the class $\W\V$ as a RKHS as in Lemma \ref{lem:rkhs} with an RBF kernel. We do the same for VAML. Further details can be found in  Appendix \ref{app:experiments}.

% Significant research effort has gone into state-of-the-art methods for offline policy optimization, dealing mostly with uncertainitly quantification \citep[]{kidambi2020morel, DeisenrothPILCO2011, Chua2018PETS, Jenner2019MBPO}. 
We input each model-learning method into MOREL \citep[]{kidambi2020morel} to examine the differences between MML, VAML and MLE. 

 \begin{algorithm}[H]
	%\begin{small}
	%\renewcommand{\thealgorithm}{}
	\caption{OPO Algorithm (based on MOREL \citep[]{kidambi2020morel}) } 
	\label{algo:meta}
	\begin{algorithmic}[1]
    	\REQUIRE $D = D_{\pi_b}P^\ast$
	    \STATE Learn an ensemble of dynamics $P_1,\ldots,P_4 \in \M$ using MML, VAML, MLE
	    \STATE Construct an $\alpha$-USAD, $U^\alpha: \State \times \A \to \{\text{TRUE},\text{FALSE}\}$ where $
	    \alpha = Median(\{ \|P_j(s,a) - s'\|_2 : j \in [1,\ldots,4], (s,a,s') \subset D\}).$ See Appendix \ref{app:morel} for the definitions.
	    \STATE Construct a pessimistic MDP $\mathcal{M}$ (see Appendix \ref{app:morel}) with $P(s,a) = \frac{1}{4} \sum_{i=1}^{4} P_i(s,a)$.
	    \STATE $\widehat{\pi} \leftarrow \text{PPO}(\mathcal{M})$ (Best of 3) \citep[]{Schulman17PPO}
	\end{algorithmic}
	%\end{small}
\end{algorithm}


\textbf{Results.} MML performs competitively with the other methods, achieving near-optimal performance as the number of trajectories increases. Unlike the other methods, MML has good performance even in the low-data regime $|D| \approx 16$, whereas other methods perform worse than $\pi_b$ with low data. This is desirable since we would like our methods to be as sample efficient as possible.

Algorithm \ref{algo:meta} forms a pessimistic MDP where a policy is penalized if it enters a state where there is disagreement between $P_1,\ldots,P_4$. Given that MML performs well in low-data, we can reason that MML produces models with support that stays within the dataset $D_{\pi_b}$ or generalize well slightly outside this set. The other models poor performance is suggestive of incorrect over-confidence outside of $D_{\pi_b}$ and PPO produces a policy which takes advantage of this.


\begin{figure}[!ht]
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/tabular_P_default.png}
% \endminipage\hfill
% \minipage{.5\textwidth}
  \includegraphics[width=\linewidth]{figs/opo_IP_edited.pdf}
% \endminipage\hfill
\vspace{-0.3in}
\caption{\textit{ Comparison of model-based approaches for OPO with function-approx (Inverted Pendulum).} \textit{MML is able to perform competitively even in low data regimes.
}}
 \label{fig:OPO}
 \vspace{-.1in}
\end{figure}

% \subsection{Learning}

% \subsubsection{Environment Description}
% We examine learning a good policy in Cartpole with a horizon of $200$ and a standard $0/1$ reward function. We collect data by running a near-perfect trained model (via TRPO) modified to take random actions with probability $1-\alpha$.  

% \subsubsection{Result}
% Figure \ref{fig:learning}(Left) illustrates the quality of policies learned over the learning iterations. What we notice is in general these methods are all fairly competitive with eachother in this environment. Different methods may converge faster than others but what we notice is that this is a function of how quickly the (log)variance converges. As we see in Figure \ref{fig:learning}(Right), after only 2 iterations the mean of MML seems to accurately predict the next state, but it takes a bit more iterations for the variance to decrease sufficiently. \clv{more} 


% \begin{figure*}[!ht]
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/learning_curve.png}
% \endminipage\hfill
% \minipage{.5\textwidth}
%   \includegraphics[width=\linewidth]{../figs/current_to_next_state.png}
% \endminipage\hfill
% \vspace{-0.1in}
% \caption{\textit{ Learning a good policy in Cartpole.} Left: \textit{The methods converge at different rates, all fall into relatively the same neighborhood.} Right: \textit{After just 2 iterations, MML already makes accurate mean predictions, but the variance is too large to learn. After many more iterations, thhe variance decreases enough that a good policy can be learned.
% }}
%  \label{fig:learning}
%  \vspace{-.1in}
% \end{figure*}

==> sec-modelfree-ope.tex <==
\section{Comparison to Model-Free OPE}
\label{sec:MFOPEComparison}
\yisong{This section feels like it should be a subsection of the previous section.}

Recent model-free OPE literature \citep[e.g.,][]{liu2018breaking, uehara2019minimax} has similar realizability assumptions to our method \yisong{reference assumption}.  \yisong{I think you need to define the rough outline of how model-free works, otherwise the subsequent discussion is not understandable to many readers.} For example, two model-free OPE methods, MQL/MWL, require either $w^{P^\ast}_{\pi}$ or $\val{\pi}{P^\ast}$ (respectively) to be realized to control the OPE error \citep[]{uehara2019minimax}.   Our model-based MML approach requires the same, in addition to terms that depend on $\M$. Computation aside, these terms are verifiable, so they do not pose a substantial theoretical challenge. 

An advantage of model-free approaches is that when both $w^{P^\ast}_{\pi}, \val{\pi}{P^\ast}$ are realized,  they return an exact OPE point estimate.  In contrast, MML additionally requires some $P \in \M$ that makes the loss zero for any $w \in \W, V \in \V$. The advantage of MML is the increased flexibility of a model, enabling OPO (Section \ref{sec:learning}) and visualization of results through simulation (leading to more transparency). 


While recent model-free OPE and our method both take a minimax approach, the classes $\W, \V, \M$ play different roles. In the model-free case, minimization is w.r.t either $\W$ or $\V$ and maximization is w.r.t the other. In our case, $\W,\V$ are on the same (maximization) team, while minimization is over $\M$. This allows us to treat $\W \times \V$ as a single unit, and represents distribution-shifted value functions. A member of this class, $E_{\text{data}}[wV]$ ($= E_{(s,a) \sim D_{\pi_b}}[\frac{\density{\pi}{P^\ast}}{D_{\pi_b}} \val{\pi}{P}(s)]$),  ties together the OPE estimate.  \yisong{Is any of this stuff that we can empirically measure or validate?  If so, we should refer to the experiments in this section.}



==> sec-related.tex <==
%!TEX root = ./icml.tex
\section{Related Work: Task and Decision Awareness}

Task-aware learning was conceived from the idea that, under misspecification of a model, the predicted dynamics should be constrained to optimize the ultimate desired problem. One of the first examples of this was a financial application \cite{bengio1997financial}. Awareness of the final task has been incorporated into stochastic dynamic programming \cite{donti2017stoch}, and adaptive optimal control (\cite{Piroddi2013NARMAX}) by adding additional feedback from the simulated performance during
model learning.

\cite{Joseph2013cartpole} introduced decision-awareness to the model-based RL community by designing an algorithm to learn a model that will optimize for expected reward. \cite{farahmand2017vaml} introduced value-aware model learning (VAML) and, its iterative version \cite{farahmand2018ivaml}, in which a model is learned to minimize error under Bellman update. This framework went on to inspire a few other algorithms that are gradient-aware and policy-aware \cite{DOro2019GAMPS, Abachi2020PAML}. Decision-awareness has also been incorporated into Deep RL in which learning involves finding models consistent with value functions. \cite{Oh2017VPN, Silver2017predictron, Luo2019framework}

Our objective function is closely related to VAML \cite{farahmand2017vaml}. 


Our approach differs from it in three details: a) b) c) 
